ViralBERT: A User Focused BERT-Based Approach to Virality Prediction

Recently, Twitter has become the social network of choice for sharing and spreading information to a multitude of users through posts called 'tweets'. Users can easily re-share these posts to other users through 'retweets', which allow information to cascade to many more users, increasing its outreach. Clearly, being able to know the extent to which a post can be retweeted has great value in advertising, influencing and other such campaigns. In this paper we propose ViralBERT, which can be used to predict the virality of tweets using content- and user-based features. We employ a method of concatenating numerical features such as hashtags and follower numbers to tweet text, and utilise two BERT modules: one for semantic representation of the combined text and numerical features, and another module purely for sentiment analysis of text, as both the information within text and it's ability to elicit an emotional response play a part in retweet proneness. We collect a dataset of 330k tweets to train ViralBERT and validate the efficacy of our model using baselines from current studies in this field. Our experiments show that our approach outperforms these baselines, with a 13% increase in both F1 Score and Accuracy compared to the best performing baseline method. We then undergo an ablation study to investigate the importance of chosen features, finding that text sentiment and follower counts, and to a lesser extent mentions and following counts, are the strongest features for the model, and that hashtag counts are detrimental to the model.

==> sections/questions.tex <==
\section*{List of questions we aim to get feedback on}

\begin{enumerate}
    % Motivation questions
    % \item Why has there been sparse recent research in this field? Why has little importance been put on being able to understand the popularity of posts of social media?
    % Dataset questions
    \item In what ways can the data collection be improved to focus on capturing specifically more viral tweets (not just tweets from users with a high number of followers)?
    % \item What is the optimal way to transform a dataset such as this one to be balanced? Was the way that was chosen the best way to do so?
    \item What is the optimal way to overcome class imbalance in a dataset such as this one? Were the best methods chosen to overcome this issue (i.e. data transformation, class boundary allocation and loss function)?
    % \item Were the best methods chosen to overcome the class imbalance in the dataset (i.e. data transformation and use of class-balanced loss function)?
    \item Were the topics that were chosen (Cryptocurrencies, TV \& Movies, Pets, Video Games, Cell Phones, COVID-19, Football and K-pop) appropriate enough to show general user usage on Twitter and would these be appropriate over time?
    % \item Would the choice of these topics mean that the models used would be outdated over time?
    % \item The Twitter API does not allow video media to be retrieved - how can we circumvent this issue if the model were to be extended to include media?
    % \item Were the retweet classes appropriate for showing virality?
    % \item Are there better class boundaries that could have been chosen given the dataset available and the need for sufficient data for each class for ML?
    % Model questions
    \item Were the baseline models chosen appropriate for comparison to \bertmodel? What other models could have been used for comparison?
    \item We experimented with adding a MLP solely for numerical features and then concatenating the output of this MLP to the output of the BERT modules running solely on tweet text before classification. This gave us worse performance that our proposed model. Why is this the case? Is our method the best way to utilise out inputs?
    % \item Was concatenating numerical features to tweet text an appropriate way to go about solving this problem?
    \item Changing the classification layers to CNNs or more complex ANNs did not improve the performance of \bertmodel. Why would this be the case? Are there any network types that could be added to improve performance?
    % \item In what ways can \bertmodel's classification layers be improved?
    \item Is the loss function selected appropriate for the task and the dataset we have used? Could there be a better one?
    \item What possible Multi-Task Learning aspects could be added to the fine-tuning of the BERT modules that would improve the performance of \bertmodel?
    % Conclusions/outcomes questions
    \item We conclude that by concatenating numerical features to text \bertmodel is able to gain context into features along with text semantics to help give better predictions. Is this a plausible explanation? % This should be investigated more into
    \item What other studies could be done to investigate the importance of features on \bertmodel or the use of its components?
    \item What are the significant factors within tweet text itself that contribute to virality (such as the use of specific rhetoric or certain expressions)?
    \item What modules or components could be added to or modified within \bertmodel to allow media to be introduced as input?
\end{enumerate}
